Separation Logic Modulo Theories

Logical reasoning about program data often requires dealing with heap structures as well as scalar data types. Recent advances in Satisfiability Modular Theory (SMT) already offer efficient procedures for dealing with scalars, yet they lack any support for dealing with heap structures. In this paper, we present an approach that integrates Separation Logic---a prominent logic for reasoning about list segments on the heap---and SMT. We follow a model-based approach that communicates aliasing among heap cells between the SMT solver and the Separation Logic reasoning part. An experimental evaluation using the Z3 solver indicates that our approach can effectively put to work the advances in SMT for dealing with heap structures. This is the first decision procedure for the combination of separation logic with SMT theories.

==> fig-mini-alg.tex <==
\begin{figure}[t]
  \centering
\begin{minipage}[t]{\linewidth}
\begin{ezcode}
 \renewcommand{\ezcodelinesep}{1pt}
  \StartLineNumbers
%
\iffalse
\Begin |fun| $\mathit{match}(\Sigma, \Sigma')$
\Begin |for each| $\fnext(x, y) \in \Sigma'$ |do|
\Begin |if| $\fnext(x, y) \in \Sigma$ |then|
\State $\Sigma \assign \Sigma - \set{\fnext(x, y)}$
\EndBegin |else|
\State |return| $\lfalse$
\End*
\End |done|
\Begin |for each| $\flseg(x, z) \in \Sigma'$ |do|
\Begin |if| $z \in \set{\mathit{addr}(S) \st S \in
\Sigma}$ |then|
\State $\Delta \assign \emptyset$
\EndBegin |else|
\State $\Delta \assign \set{\flseg(w, y) \in \Sigma \st y \neq z}$
\State $\Sigma \assign \Sigma - \Delta$
\End $\mathit{curr} \assign x$
\Begin |while| $\mathit{curr} \neq z$ |do|
\Begin |if| exits $f(\mathit{curr}, y) \in \Sigma$ |then|
\State $\Sigma \assign \Sigma - \set{f(\mathit{curr}, y)}$
\State $\mathit{curr} \assign y$
\EndBegin |else|
\State |return| $\lfalse$
\End*
\End |done|
\State $\Sigma \assign \Sigma \cup \Delta$
\End |done|
\State |return| $\Sigma = \emptyset$
\End |end|
\fi
%
\medskip
\Begin |fun| $\mathit{prove}(\Pi \land \Sigma \limp \Pi' \land \Sigma')$
\State $\Gamma \assign 
  \begin{array}[t]{@{}l@{}}
    \Pi \mathrel{\land} \wfOf{\Sigma}
    \iffalse
    \bigwedge_{S\neq T \in \Sigma}
    (\begin{array}[t]{@{}l@{}}
      \mathit{addr}(S) \feq \mathit{addr}(T) 
      \limp  \\[\jot] 
      \mathit{empty}(S) \lor \mathit{empty}(T))
    \end{array}
    \fi
  \end{array}
  $
  \Begin |while| $\mathit{sat}(\Gamma)$ |do|
  \State $I \assign \mathit{solve}(\Gamma)$
  \State $\sigma \assign \lambda x\in V\,.\ \text{min}_\prec \set{ y
    \in V \st I(x) = I(y)}$
  \State $\varphi \assign 
  \begin{array}[t]{@{}l@{}}
    \mathit{distinct}(\set{\sigma(x) \st x\in V}) \mathrel{\land}\\[\jot]
    \bigwedge \set{ x \feq \sigma(x) \st x \in V}
  \end{array}
  $
  \Begin |if| $(I \models \Pi') \land \mathit{match}(\Sigma\sigma, \Sigma'\sigma)$ |then|
  \State $\Gamma \assign \Gamma \land \neg \varphi$
  \EndBegin |else|
  \State |return| $\finvalid$
  \End*
  \End |done|
  \State |return| $\fvalid$
  \End |end.|
\end{ezcode}
\end{minipage}
  \caption{Mini algorithm.}
  \label{fig-mini-alg}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> fig-symb-alg.tex <==
Hybrid version

\begin{ezcode}
 \renewcommand{\ezcodelinesep}{1pt}
\StartLineNumbers
\Begin |function| $\Match(s, U, \hat\Sigma, \Sigma, \Sigma')$
  \Begin |if| exists $S \in \Sigma$ s.t.\ $s \models \Empty(S)$ |then|
    \State |return| $\Match(s, \hat\Sigma, U \land \Empty(S), \Sigma \setminus S, \Sigma')$
  \EndBegin |if| exists $S' \in \Sigma'$ s.t.\ $s \models
  \Empty(S')$ |then|
    \State |return| $\Match(s, \hat\Sigma, U \land \Empty(S'), \Sigma, \Sigma' \setminus S')$
  \EndBegin |if| exists $S \in \Sigma$ and $S' \in \Sigma'$ s.t.\ %uch that
    $s \models \UnfoldCheck(\hat\Sigma, S, S')$ 
 |then|
      \State |return|
      $\Match(
        s, \hat\Sigma, %\\[\jot]
      \begin{array}[t]{@{}l@{}}
        U \land \UnfoldCheck(\hat\Sigma, S, S'),\\ [\jot]
        \Sigma \setminus S, \UnfoldStep(S, S') \ast (\Sigma' \setminus S'))
      \end{array}
      $
  \EndBegin |return| $(\Sigma \neq \emptyset) \land (\Sigma' \neq
  \emptyset) \land U$
  \End*
  \End*
\end{ezcode}

Explicit version

\begin{ezcode}
 \renewcommand{\ezcodelinesep}{1pt}
\StartLineNumbers
\Begin |function| $\Match(s, \hat\Sigma, \Sigma, \Sigma')$
  \Begin |if| exists $S \in \Sigma$ s.t.\ $s \models \Empty(S)$ |then|
    \State |return| $\Match(s, \hat\Sigma, \Sigma \setminus S, \Sigma')$
  \EndBegin |if| exists $S' \in \Sigma'$ s.t.\ $s \models
  \Empty(S')$ |then|
    \State |return| $\Match(s, \hat\Sigma, \Sigma, \Sigma' \setminus S')$
  \EndBegin |if| exists $S \in \Sigma$ and $S' \in \Sigma'$ s.t.\ %uch that
    $s \models \UnfoldCheck(\hat\Sigma, S, S')$ 
 |then|
      \State |return|
      $\Match(
        s, \hat\Sigma, 
        \Sigma \setminus S, \UnfoldStep(S, S') \ast (\Sigma' \setminus S'))
      $
  \EndBegin |return| $(\Sigma \neq \emptyset) \land (\Sigma' \neq \emptyset)$
\end{ezcode}

\endinput

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> general-alg.tex <==
\begin{ezcode}
\StartLineNumbers
\Begin |function| $\Unfolding(s, \Sigma_0, \Sigma'_0)$
  \State \emph{\textless\ assumes: $s \models W(\Sigma_0)$ \textgreater}
  \State $\tuple{U, \Sigma, \Sigma', \hat\Sigma} \assign \tuple{\smodel{\Sigma_0}, \Sigma_0, \Sigma'_0, \femp}$ \label{unf:init}
  \Begin |for each| $S$ |in| $\Sigma$ |such that| $s \models \Empty(S)$ |do| \label{unf:l_empty}
    \State $U \assign U \land \Empty(S)$
    \State |move| $S$ |from| $\Sigma$ |into| $\hat\Sigma$
  \End*
  \Begin |while| $\Sigma' \neq \femp$ |with some| $S'$ in $\Sigma'$ |do| \label{unf:pick_sp}
    \Begin |if| $s \models \Empty(S')$ |then|
      \State $U \assign U \land \Empty(S')$ \label{unf:r_empty}
      \State |remove| $S'$ |from| $\Sigma'$
    \EndBegin |else if| $s \models \NonEmpty(S')$ |then|
      \Begin |if there is a| $S$ |in| $\Sigma$ |such that| $s \models S \intersects S'$ |do|
        \State $\tuple{\Sigma'',C} \assign \UnfoldStep(S, S', \Sigma_0)$
        \State if $s \not\models C$ |then return| $\ffalse$ \label{unf:unfold}
        \State $U \assign S \intersects S' \land C$
        \State |replace| $S'$ |in| $\Sigma'$ |with| $\Sigma''$
        \State |move| $S$ |from| $\Sigma$ |into| $\hat\Sigma$
      \EndBegin |else|
        \State |return| $\ffalse$ \label{unf:not_paired}
      \End*
    \EndBegin |else|
      \State |return| $\ffalse$ \label{unf:not_satisfied}
    \End*
  \End*
  \Begin |if| $\Sigma \neq \femp$ |then|
    \State |return| $\ffalse$ \label{unf:not_exhausted}
  \EndBegin |else|
    \State |return| $U$ \label{unf:success}
  \End*
\End*
\end{ezcode}


==> inductpred.tex <==
\def\RowsA{}
\def\RowsB{}
\def\Multi{\multicolumn{5}{l}}
\newcommand\InductivePred[8]{%
  \appto\RowsA{#2 & #3 & #4 & #5 & #6 & \text{#8} \\}
  \appto\RowsB{#2 & \Multi{#7} \\}
}
%
\InductivePred{Empty heap}
  {\femp}{\emptyset}
  {\ftrue}
  {\ffalse}
  {\text{---}}
  {\text{---}}
  {}
%
\InductivePred{Allocated record}
  {x \mapsto \rho}{\set{x}}
  {\ffalse}
  {\ftrue}
  {\cell{x \mapsto \rho}}
  {\cell{x \mapsto \rho}}
  {}
%
\InductivePred{Acylcic list segment}
  {\flseg(x,z)}{\set{x}}
  {x \feq z}
  {x \fneq z}
  {\exists y \dt \lsegcell{x}{y} \ast \flseg(y, z)}
  {\lsegcell{x}{z}}
  {\cite{Berdine:2005fk}}
%
\InductivePred{Acyclic list segment with length}
  {\flseg(x,z;k)}{\set{x}}
  {x \feq z \land k \feq 0}
  {x \fneq z \land k > 0}
  {\exists y \dt \lsegcell{x}{y} \ast \flseg(y, z; k - 1)}
  {\lsegcell{x}{y_1} \ast \dots \ast \lsegcell{y_{k-2}}{y_{k-1}} \ast \lsegcell{y_{k-1}}{z}}
  {\cite{Magill:2007vn}}
%
\InductivePred{Cyclic list segment}
  {\fclseg(x,z)}{\set{x}}
  {e \land x \feq z}
  {\lnot e}
  {\exists y \dt \lsegcell{x}{y} \ast \fclseg(y, z)}
  {\lsegcell{x}{z}}
  {\cite{Berdine:2005kx}}
%
\InductivePred{Doubly-linked list}
  {\fdlseg(x, z, x', z')}{\set{x,z'}}
  {x \feq z \land x' \feq z'}
  {x \fneq z \land x' \fneq z'}
  {\exists y \dt \dlsegcell{x}{y}{x'} \ast \fdlseg(y,z,x,z')}
  {\dlsegcell{x}{z'}{x'}\ast\dlsegcell{z'}{z}{x}}
  {\cite{Berdine:2006uq}}
%
\InductivePred{Tree}
  {\ftree(x)}{\set{x}}
  {x \feq \fnil}
  {x \fneq \fnil}
  {\exists y, z \dt \treecell{x}{y}{z} \ast \ftree(y) \ast \ftree(z)}
  {\treecell{x}{\fnil}{\fnil}}
  {\cite{Berdine:2005fk}}
%
\begin{array}{l@{\qquad}l@{\qquad}l@{\qquad}l@{\qquad}l@{\qquad}l}
S & \Alloc(S) & \Empty(S) & \NonEmpty(S) & \Induct(S) \\\hline
\RowsA%[2ex]
%S & \Multi{\Wit(S)} \\\hline
%\RowsB
\end{array}


==> judgement.tex <==
\newcommand\UnfRule[2]{
  \begin{array}{l@{{}\land{}}c@{{}\ast{}}c@{{}\lthen{}}c@{{}\equiv{}}c@{{}\ast{}}c}
  \UnfRow#1\hline
  \UnfRow#2
  \end{array}
}
%
\newcommand\UnfRow[4]{
  s \Cons \Pi_0 \land \Land{\Pi}{#1} & 
  \Ast{\Sigma'}{#2}                  & 
  \Ast{#3}{\hat\Sigma}               &
  \Sigma'_0 \Cons \Sigma_0           &
  \Ast{\Sigma}{#4}                   &
  \Ast{#3}{\hat\Sigma}               \\
}
%
\begin{gather*}
\UnfRule
  {{}{}{}{S}}
  {{\Empty(S)}{}{S}{}}\; \text{emp-I} \\[4ex]
\UnfRule
  {{}{S'}{}{}}
  {{\Empty(S')}{}{}{}}\; \text{emp-E} \\[4ex]
\UnfRule
  {{}{S'}{}{S}}
  {{(\Alloc(S') \cap \Alloc(S)) \land C}{S''}{S}{}}\; \text{unfold}
\end{gather*}
\endinput


==> unfold-steps.tex <==
\begin{gather*}
\Step{\State{}{}{S}{}}{\State{E}{S}{}{}}{E} \qquad
\Step{\State{}{}{}{S'}}{\State{E'}{}{}{}}{E'} \qquad
\Step{\State{}{}{*}{*}}{U}{\ftrue} \\[2ex]
\Step{\State{}{}{}{S'}}{\ffalse}{\lnot N' \land \lnot E'} \qquad
\Step{\State{}{}{}{S'}}{\ffalse}{N' \land D'} \qquad
\Step{\State{}{}{S}{*}}{\ffalse}{N} \\[2ex]
\Step{\State{}{}{S}{S'}}{\State{\lnot D \land C}{S}{}{\Sigma''}}{\lnot D \land C} \qquad
\Step{\State{}{}{S}{S'}}{\ffalse}{\lnot D \land \lnot C}
\end{gather*}
\medskip
\hrule
\footnotesize
\begin{align*}
E  &= \Empty(S) &
N  &= \NonEmpty(S) &
D  &= \Disjoint(S, S') &
C  &= \UnfoldCheck(S, S', \Sigma_0) \\
E' &= \Empty(S') &
N' &= \NonEmpty(S') &
D' &= \Disjoint(\Sigma, S') &
\Sigma'' &= \UnfoldStep(S, S')
\end{align*}

